Towards ISAC RIS-Enabled Passive Radar Target Localization

Incorporating integrated sensing and communication capabilities into forthcoming 6G wireless networks is crucial for achieving seamless synchronization between the digital and physical worlds. The following paper focuses on a scenario where a passive radar (PR) is subject to weak line-of-sight signals of opportunity, emanating from an access point and subsequently reflecting off targets, ultimately reaching the PR. Furthermore, a normalized least mean squares method is presented for jointly detecting the number of targets and estimating target angles of arrival (AoAs). The algorithm iteratively adjusts the steering vector estimates to minimize a suitable error cost function, while the target AoAs are identified via a peak-finding search conducted on the resulted power spectrum. Simulation results show the capabilities of the proposed localization method, as well as a 14 dB dynamic range reduction that can be achieved at the PR.

==> sections/isac-metrics.tex <==
%% Mutual information 
\Ac{MI} is a measure of the amount of information that one random variable incorporates about another random variable, i.e. how relevant both variables are to each other.
%% Comm 
For that, we make use of the \ac{MI} as a performance criterion for communication 
For communications, the mutual information between the $k^{th}$ channel and the received \ac{DL} signal at the $k^{th}$ user and can be written as
\begin{equation}
	\mathcal{I}(\mathbf{y}_k; \mathbf{h}_k)
	=
	h(\mathbf{y}_k)
	-
	h(\mathbf{y}_k \vert \mathbf{h}_k ).
\end{equation}
As an exact closed form solution may seem difficult to optimize, instead, we resort to the following proposition, which aims at approximating $\mathcal{I}(\mathbf{y}_k; \mathbf{h}_k)$ as follows

\textbf{Proposition 1}: \textit{For a given pilot matrix $\mathbf{\Phi}$, the mutual information between $\mathbf{h}_k$ and $\mathbf{y}_k$ can be approximated as $\mathcal{I}(\mathbf{y}_k; \mathbf{h}_k) \simeq  \mathcal{M}_k^{\tt{comm}}(\mathbf{\Phi})$ where}
\begin{equation}
\label{eq:M-comm-k}
	\mathcal{M}_k^{\tt{comm}}(\mathbf{\Phi}) \triangleq
	- \log \Big(\sum\nolimits_{n=1}^{N_k}  \frac{\alpha_{k,n} e^{-\beta_{k,n}(\mathbf{\Phi})}}{\det (\mathbf{\Sigma}_{k,n}(\mathbf{\Phi})) } \Big)  +
	\tt{cnst},
\end{equation} 
\textit{and}
\begin{align}
	\label{beta-expression}
	\beta_{k,n}(\mathbf{\Phi}) &= \bar{\mathbf{\mu}}_{k,n}^H\mathbf{\Phi}^H \mathbf{\Sigma}_{k,n}^{-1}(\mathbf{\Phi})\mathbf{\Phi}\bar{\mathbf{\mu}}_{k,n}, \\
	\label{eq:mu_bar}
	\bar{\mathbf{\mu}}_{k,n} &=\sum\nolimits_{n' = 1}^{N_k}\alpha_{k,n'}\mathbf{\mu}_{k,n'} - \mathbf{\mu}_{k,n}, \\
	\label{eq:Sigma_Phi}
	\mathbf{\Sigma}_{k,n}(\mathbf{\Phi}) &=  \mathbf{\Phi}\mathbf{R}_{k,n}\mathbf{\Phi}^H + \sigma_k^2 \mathbf{I}_L.
\end{align}
\textit{Furthermore, ${\tt{cnst}}$ is a term independent of $\mathbf{\Phi}$.}

\textbf{Proof}: See \cite{bazzi2023mutual}.

%% Sensing
Hypothesis testing is a well-known approach towards target detection in radar problems. 
For instance, the work in \cite{831834} derives optimal waveforms via hypothesis testing in the presence of clutter interference, which was iteratively solved. Indeed, one can reformulate \eqref{eq:yr} through vectorization as
\begin{equation}
\label{eq:Hypothesis-test-1}
	\begin{cases}
		\mathcal{H}_0: \qquad \mathbf{y}_r =  \mathbf{c} + \mathbf{n}_r, \\ 
		\mathcal{H}_1: \qquad \mathbf{y}_r = \mathbf{d} +\mathbf{c} + \mathbf{n}_r.
	\end{cases}
\end{equation}
In the above, we have $\mathbf{y}_r = \ve(\mathbf{Y}_r)$, $\mathbf{n}_r = \ve(\mathbf{N}_r)$, $\mathbf{c} \triangleq \sum\nolimits_{i=1}^Q \gamma_i \mathbf{\mu}_i$ and $\mathbf{d} \triangleq \gamma_0 \mathbf{\mu}_0$, where 
\begin{equation}
 	\mathbf{\mu}_i = \ve(\mathbf{a}_{N_r}(\theta_i)\mathbf{a}_{N_t}^T(\theta_i)\mathbf{\Phi}^T ),
\end{equation}
We can conveniently re-express \eqref{eq:Hypothesis-test-1} as follows
\begin{equation}
\label{eq:Hypothesis-test-2}
	\begin{cases}
		\mathcal{H}_0: \ \mathbf{z} \sim \mathcal{CN}(\mathbf{0},\mathbf{I}), \\ 
		\mathcal{H}_1: \ \mathbf{z} \sim \mathcal{CN}(\mathbf{0},(\mathbf{R}_{\mathbf{cc}} + \sigma_r^2 \mathbf{I})^{-\frac{1}{2}}\mathbf{R}_{\mathbf{dd}}(\mathbf{R}_{\mathbf{cc}} + \sigma_r^2 \mathbf{I})^{-\frac{1}{2}} + \mathbf{I}),
	\end{cases}
\end{equation}
where $\mathbf{R}_{\mathbf{cc}} = \mathbb{E}( \mathbf{c} \mathbf{c}^H)$ and $\mathbf{R}_{\mathbf{dd}} = \mathbb{E}( \mathbf{d} \mathbf{d}^H)$. 
Also, $\mathbf{z} = (\mathbf{R}_{\mathbf{cc}} + \sigma_r^2 \mathbf{I})^{-\frac{1}{2}}\mathbf{y}_r$ is a pre-whitened version of $\mathbf{y}_r$. 
Interestingly, we can relate the performance of the hypothesis testing problem in \eqref{eq:Hypothesis-test-1} (equivalently \eqref{eq:Hypothesis-test-2}) to the \ac{MI} between the observed data and the parameters of interest, namely $\mathcal{I}(\mathbf{Y}_r;\mathbf{\Theta},\mathbf{\nu} \vert \mathbf{\Phi})$ \cite{259642}. However, dealing with the direct form of $\mathcal{I}(\mathbf{Y}_r;\mathbf{\Theta},\mathbf{\nu} \vert \mathbf{\Phi})$ can be difficult to optimize, therefore, we resort to an approximate form of the sensing \ac{MI}. For this, we have the following proposition

\textbf{Proposition 2}: \textit{For a given pilot matrix $\mathbf{\Phi}$ and large  $N_r$, the \ac{MI} related to the hypothesis testing problem in \eqref{eq:Hypothesis-test-1} (equivalently \eqref{eq:Hypothesis-test-2}) can be approximated as $\mathcal{I}(\mathbf{Y}_r;\mathbf{\Theta},\mathbf{\nu} \vert \mathbf{\Phi}) \simeq \mathcal{M}^{\tt{sense}}(\mathbf{\Phi})$, where}
\begin{equation*}
	\mathcal{M}^{\tt{sense}}(\mathbf{\Phi}) \triangleq \log (1+ \frac{\nu_0}{\sigma_r^2 } \Vert \mathbf{\mu}_0 \Vert^2 -\frac{\nu_0}{\sigma_r^2 }\sum\limits_{i=1}^Q  \frac{  \nu_i\vert\mathbf{\mu}_0^H\mathbf{\mu}_i \vert^2}{\sigma_r^2 + \nu_i \Vert \mathbf{\mu}_i \Vert^2}).
\end{equation*}

\textbf{Proof}: See \cite{bazzi2023mutual}.

Thanks to the approximate \ac{MI} closed form expressions in both propositions, we can now design an optimization framework tailored to maximize both communication and sensing \acp{MI} in order to enhance target detection, as well as communication performances.





==> sections/optimized-isac-pilots.tex <==
\begin{figure}[t]
	\centering
	\ctikzfig{./figures/tikzPlayground/PGD}
	\caption{An illustration demonstrating the convergence of the pilot matrix via \ac{PGD} for \ac{ISAC} pilot-design. The global maximum of $\mathcal{M}^{\tt{ISAC}}(\mathbf{\Phi})$ is $\mathbf{\Phi}^{\tt{opt}}$.}
	\label{fig:PGD}
\end{figure}
A fundamental, yet important, question to ask is whether one can generate orthogonal pilots capable of performing \ac{ISAC} functionalities. In other words, \textit{can pilots be good enough to perform target detection, while simultaneously be reliably used for channel estimation to carry out further communication tasks ?}
In this section, we formulate a \ac{MOOP} with intentions of affirming the aforementioned question.
Based on this, we design the following $K + 1$ dimensional \ac{MOOP}
\begin{equation}
	\label{eq:MOOP1}
\begin{aligned}
(\mathcal{P}_{\tt{MOOP}}):
\begin{cases}
\max\limits_{\mathbf{\Phi} }&  \begin{bmatrix}
	\mathcal{M}_1^{\tt{comm}}(\mathbf{\Phi}),
	 \ldots,
	 \mathcal{M}_K^{\tt{comm}}(\mathbf{\Phi}), 
	 \mathcal{M}^{\tt{sense}}(\mathbf{\Phi})
\end{bmatrix} \\
\textrm{s.t.}
 & \mathbf{\Phi}\mathbf{\Phi}^H = \mathbf{I},
\end{cases}
\end{aligned}
\end{equation}
which aims at maximizing all the involved communication and sensing \acp{MI}.
The proposed \ac{MOOP} is very hard to solve due to the multi-dimensional objective function nature and prone to be trapped by local optima due to its complicated  nonlinear and non-convex nature of the underlying functions.
Multi-objective evolutionary algorithms and metaheuristics are one approach, however they suffer from high computational cost in realtime \cite{luna2016distributed}.
In order to overcome this, and in order to balance the conflicting metrics between sensing and communications, we resort to a linearization technique, also referred to as the \textit{a priori method} \cite{6924852}.
Therefore, instead of considering \eqref{eq:MOOP1}, we scalarize the cost to obtain
\begin{equation}
	\label{eq:scalarization1}
\begin{aligned}
(\mathcal{P}):
\begin{cases}
\max\limits_{\mathbf{\Phi} }&  \mathcal{M}^{\tt{ISAC}}(\mathbf{\Phi}) \\
\textrm{s.t.}
 & \mathbf{\Phi}\mathbf{\Phi}^H = \mathbf{I}.
\end{cases}
\end{aligned}
\end{equation}
where 
$\mathcal{M}^{\tt{ISAC}}(\mathbf{\Phi}) \triangleq \rho \mathcal{M}^{\tt{comm}}(\mathbf{\Phi}) + (1-\rho)\mathcal{M}^{\tt{sense}}(\mathbf{\Phi}) $, 
$\mathcal{M}^{\tt{comm}}(\mathbf{\Phi}) = \sum_k w_k \mathcal{M}_k^{\tt{comm}}(\mathbf{\Phi})$ and $\sum_k w_k = 1$. 
Indeed, the weights $w_k$ are positive, and as highlighted in \cite{6924852}, one should be careful when interpreting relative priorities. 
This is because the objectives can be operating on contrasting scales, which may affect the choice of weights.
As far as our \ac{ISAC} cost is concerned, the objectives are all expressed in bits, as they are all \ac{MI}-based, therefore the scales are more or less scale-compatible.  


We propose a \ac{PGD} algorithm to optimize the pilots $\mathbf{\Phi}$ that maximize $\mathcal{M}^{\tt{ISAC}}(\mathbf{\Phi})$ in \eqref{eq:scalarization1} under the orthogonal constraint. 
More specifically, the designed \ac{PGD} performs the following updates
\begin{align}
	\label{eq:GD-step}
	\mathbf{Z}_{t+1} 
	&=
	\mathbf{\Phi}_{t}
	+
	\gamma
	\nabla_{\mathbf{\Phi}}
	\mathcal{M}^{\tt{ISAC}}(\mathbf{\Phi})
	\Big\vert _{\mathbf{\Phi} = \mathbf{\Phi}_{t}}, \\
	\label{eq:project-step}
	\mathbf{\Phi}_{t+1}
	&=
	\mathbf{\pi}(\mathbf{Z}_{t+1} ),
\end{align}
where 
\begin{equation}
	\label{eq:GD-project}
	\mathbf{\pi}(\mathbf{Y})
	=
	\argmin_{\mathbf{X} \in {\tt{St}}(L,N_t)}
	\Vert
	\mathbf{X}
	-
	\mathbf{Y}
	\Vert^2_F.
\end{equation}
where ${\tt{St}}(N_t,L) = \lbrace \mathbf{X} \in \mathbb{C}^{L 
\times N_t}: \mathbf{X}\mathbf{X}^H = \mathbf{I}_{L}\rbrace$ is the Stiefel manifold. 
Note that for the case of $N_t > L$, $\mathbf{\pi}(\mathbf{Y}) = \mathbf{U}\mathbf{I}_{L,N_t}\mathbf{V}^H$, where $\mathbf{I}_{L,N_t} \in \mathbb{R}^{L \times N_t}$ is a rectangular diagonal matrix with all of its diagonal entries set to $1$. 
Also $\mathbf{Y} = \mathbf{U}\mathbf{\Lambda}\mathbf{V}^H$ represents the \ac{SVD} operation. 
Observe that \eqref{eq:GD-step} performs a descent step and \eqref{eq:project-step} projects the current point, which is not necessarily feasible, onto the closest point that lies within the feasible set, i.e. the Stiefel manifold.
In this way, a \ac{PGD} update ensures to output an orthogonal pilot, while optimizing the \ac{MI}-based \ac{ISAC} cost.
In \cite{bazzi2023mutual}, we analyze the convergence behaviour of the proposed \ac{PGD} method and show that, even though the underlying functions are not convex, the \ac{PGD} iterations are guaranteed to converge to a satisfactory pilot matrix.
Furthermore, the gradient term appearing in equation \eqref{eq:GD-step} is 
\begin{equation}
\label{eq:dMISAC}
\begin{split}
	\nabla_{\mathbf{\Phi}}
	\mathcal{M}^{\tt{ISAC}}(\mathbf{\Phi})
	&=
	\rho \sum_k w_k \nabla_{\mathbf{\Phi}}\mathcal{M}_k^{\tt{comm}}(\mathbf{\Phi}) \\
	&+ (1-\rho)\nabla_{\mathbf{\Phi}}\mathcal{M}^{\tt{sense}}(\mathbf{\Phi}),
\end{split}
\end{equation}
In \cite{bazzi2023mutual}, we show that the above gradients are given in closed form as follows
\begin{equation}
\label{eq:dMsense}
	\nabla_{\mathbf{\Phi}_l}\mathcal{M}^{\tt{sense}}(\mathbf{\Phi}) =  
	\frac{g_0(\mathbf{\Phi}) - \sum_{i=1}^Q g_i(\mathbf{\Phi})}{1+ \frac{\nu_0}{\sigma_r^2 } \Vert \mathbf{\mu}_0 \Vert^2 -
	\frac{\nu_0}{\sigma_r^2 }\sum\nolimits_{i=1}^Q  \frac{  \nu_i\vert\mathbf{\mu}_0^H\mathbf{\mu}_i \vert^2}{\sigma_r^2 + \nu_i \Vert \mathbf{\mu}_i \Vert^2}}.
\end{equation}
where $g_0(\mathbf{\Phi}) = \frac{2\nu_0}{\sigma_r^2 }\mathbf{A}^H(\theta_i)\mathbf{A}(\theta_i)\mathbf{\Phi}_l$ and $g_i = g_i^{(1)} + g_i^{(2)}$, where $g_i^{(1)}$ and $g_i^{(2)}$ are given as follows
\begin{align}
	g_i^{(1)}(\mathbf{\Phi}) &= \xi_i\big( \mathbf{A}^H(\theta_0)\mathbf{A}(\theta_i) + \mathbf{A}^H(\theta_i)\mathbf{A}(\theta_0) \big)\mathbf{\Phi}_l, \\
	g_i^{(2)}(\mathbf{\Phi}) &= - \varphi_i \mathbf{A}^H(\theta_i)\mathbf{A}(\theta_i)\mathbf{\Phi}_l,
\end{align}
where $\xi_i = \frac{2\nu_i \Re[\mathbf{\mu}_0^H \mathbf{\mu}_i]}{(\sigma_r^2 + \nu_i \Vert \mathbf{\mu}_i \Vert^2)}$ and 
$\varphi_i = \frac{2\nu_i^2 \vert\mathbf{\mu}_0^H\mathbf{\mu}_i \vert^2 }{(\sigma_r^2 + \nu_i \Vert \mathbf{\mu}_i \Vert^2)^2}$.
In addition, the gradient of $\mathcal{M}_k^{\tt{comm}}(\mathbf{\Phi}) $ with respect to $\mathbf{\Phi}$ can be written as	
\begin{equation}
\label{eq:dMcomm}
\begin{split}
	\nabla_{\mathbf{\Phi}}\mathcal{M}_k^{\tt{comm}}(\mathbf{\Phi}) 
	&=
\frac{2}{\omega_k(\mathbf{\Phi})}
	 \sum_{n=1}^{N_k}
	 d_{k,n}
	 \Bigg\lbrace
	 \mathbf{\Sigma}^{-1}_{k,n}(\mathbf{\Phi})
	 \mathbf{\Phi}
	 \mathbf{R}_{k,n} 
	  \\ & 
-	\mathbf{R}_{k,n}\mathbf{\Phi}^H \mathbf{\Sigma}^{-1}_{k,n}(\mathbf{\Phi}) \mathbf{\Phi} \bar{\mathbf{\mu}}_{k,n}\bar{\mathbf{\mu}}_{k,n}^H \mathbf{\Phi}^H  \mathbf{\Sigma}^{-1}_{k,n}(\mathbf{\Phi}) \\ &
+ 	 \bar{\mathbf{\mu}}_{k,n}\bar{\mathbf{\mu}}_{k,n}^H\mathbf{\Phi}^H \mathbf{\Sigma}^{-1}_{k,n}(\mathbf{\Phi}) 
	 \Bigg\rbrace,
\end{split}
\end{equation}
where $\omega_k(\mathbf{\Phi}) = \sum_{n=1}^{N_k}  d_{k,n}$ and $d_{k,n} = \frac{\alpha_{k,n}e^{-\beta_{k,n}(\mathbf{\Phi})} }{\det (\mathbf{\Sigma}_{k,n}(\mathbf{\Phi}))}$. In addition, $\mathbf{A}(\theta) = \mathbf{a}(\theta)\mathbf{a}^H(\theta) $.
Using \eqref{eq:dMsense} and \eqref{eq:dMcomm} in \eqref{eq:dMISAC}, one can execute the \ac{PGD} step in \eqref{eq:GD-step}.



  
